Moving Window Network Coding in Cooperative Multicast (v1)

Cooperative multicast is an effective solution to address the bottleneck problem of single-hop broadcast in wireless networks. By incorporating with the random linear network coding technique, the existing schemes can reduce the retransmission overhead significantly. However, the receivers may incur large decoding delay and complexity due to the batch decoding scheme. In addition, the dependency on the explicit feedback leads to scalability problem in larger networks. In this paper, a cooperative multicast protocol named MWNCast is proposed based on a novel moving window network coding technique. We prove three properties of the proposed scheme. Firstly, without explicit feedback, MWNCast can approach the cooperative capacity with the packet loss probability dropping almost exponentially with the increase of window size. Secondly, the average decoding delay of a receiver is on the order of $O(\frac{1}{(1-\rho)^2})$ with respect to its traffic intensity $\rho$. Thirdly, MWNCast can achieve the linear decoding complexity of $O(W)$ with respect to the window size $W$. Simulation results show that MWNCast outperforms the existing schemes by achieving better tradeoff between the throughput and decoding delay, meanwhile keeping the packet loss probability and decoding complexity at a very low levelwithout explicit feedback.

==> sect4-old.tex <==
\section{Design of MWNCast}\label{sec:design}
In this section, we propose MWNCast, a cooperative multicast
protocol based on MWNC technique. Before elaborating on the details
of the protocol, we provide an overview of MWNCast with a simple example.

\subsection{Overview of MWNCast}
Consider a simple example as shown in Fig. \ref{fig:example}(a),
which contains three receivers, the number on each link indicates
the corresponding PRP. For plain broadcast, it is easy to see the
bottleneck throughput of the system is $0.4$ incurred by client
$R_3$, which require twice of the time to receive the same amount of
information as that of clients $R_1$ and $R_2$. In other words, one
half of the time is wasted for clients $R_1$ and $R_2$ since the
information sent by the source is not innovative to these two receivers
after they have received the required data. On the other hand, if
these two clients have packets that are not received by client
$R_3$, we can let one of them to relay the packets to client 3 on
behalf of the source on a different channel, while the other client can
continue receiving data from the base station. Ideally, if clients
$R_1$ and $R_2$ only spend 3/4 of their time to receive from the source,
and contribute the rest 1/4 of their time to serve client $R_3$ in
turn, then the maximum achievable throughput for them is $0.8 \times
\frac{3}{4}=0.6$. Meanwhile, client $R_3$ can receive data
alternately from clients $R_1$ and $R_2$ in half of its time, and
from the source in the rest half time, so its achievable throughput is
also $\frac{1}{2}\times 0.8+\frac{1}{2}\times 0.4 = 0.6$. This
cooperation strategy is shown in Fig. \ref{fig:example}(b), which
can increase the multicast capacity by $50\%$.

The key to the success of this cooperative strategy is scheduling
the relay transmissions, that is, to determine which set of relay
node should transmit at a specific time slot. To this end, we adopt
a stochastic scheduling method, which works as follows. At the
beginning of each time slot, the source generates a random variable $x$
uniformly distributed in $[0,1]$. If $0\le x<\frac{1}{4}$, then
$R_1$ is selected to relay the data to $R_3$, while $R_2$ keeps
receiving from the source. If $\frac{1}{4}\le x<\frac{1}{2}$, the roles
of $R_1$ and $R_2$ are exchanged. Otherwise, only the source transmits
and all clients receive information from it. This scheduling
decision is broadcasted to all relays. Each second-hop receiver
always receives from the best transmitter (the source or a relay). An
example of the scheduling sequences is shown in Fig.
\ref{fig:example}(c).

Once the schedule gets confirmed, MWNC is operated on the source and the
selected relays. The moving speed $V$ of coding window should be
within the network capacity ($0.6$ for this example). Define the
packets ranging from $\lceil V\cdot t \rceil -W +1$ to $\lceil
V\cdot t \rceil$ as the expected window at time $t$. When the
transmission begins, the source simply sends a random combination of the
packets in the expected window on its own channel, while the
selected relay sends a specifically coded symbol on the relaying
channel. In specific, this coded symbol is generated from a batch of
packets (the most close to the expected window in the relay's
buffer), including the newly decoded packets and the combination of
undecoded packets (e.g., $p_{10}$, $p_{11}$, and $p_{12}$ in Fig.
\ref{fig:example}(d)).  By overhearing the transmissions from the source
and the relay, a second-hop $receiver$ can attempt to decode the
original packets with Gauss-Jordan elimination approach.

%. A snapshot of MWNCast ($K=2,V=0.5, W=3$) at $t=25$ is shown in
%Fig. \ref{fig:example}(d), whereby in the beginning the source
%broadcasts the channel allocation decision, then all other stations
%adjust their channel accordingly. After confirming it's not its turn
%to relay, $R_1$ shifts its radio to the source's channel while $R_3$
%listens on the relay's channel for better transmission quality. MWNC
%operates on the source and the relays, but its process at the relay
%stations requires more explanations: the current relay $R_2$
%generates the coded symbol from a batch of packets most close to the
%expected window. As shown in Fig. \ref{fig:example}, it mixes two
%undecoded packet combinations in the buffer with random
%coefficients.

%\begin{figure}[t]
%\centering
%\includegraphics[width=3.6in]{figure/broadcast_example.eps}
%  \caption{An simple example of MWNCast}
%  \label{fig:broadcast_example}
%\end{figure}

\begin{figure}[t]
\centering
\subfigure[Topology]{
 \includegraphics[width=0.63in]{figure/topology.eps}}
\subfigure[MWNCast]{
  \includegraphics[width=0.62in]{figure/MWNCast.eps}}
\subfigure[Scheduling]{
  \includegraphics[width=0.8in]{figure/schedule.eps}}
\subfigure[Coding]{
  \includegraphics[width=0.95in]{figure/Coding.eps}}
  \caption{A simple example of MWNCast}
  \label{fig:example}
\end{figure}


\subsection{MWNCast protocol}
In this subsection, we discuss the details of MWNCast protocol. As
we have explained how to implement MWNC in a cooperative scenario,
in the following we mainly focus on illustrating the cooperative
scheduling utilized in MWNCast, which can be decomposed into three
modules, namely the selection of relay nodes, the allocation of
relay time, and the online scheduling of relay transmissions.


\subsubsection{Selection of relay nodes} The ultimate objective of
MWNCast is to alleviate the bottleneck and maximize the multicast
capacity through the cooperation of relay clients. To this end, we
propose a procedure to search for a set of candidate relay nodes
that can achieve the maximum capacity. The basic idea is as follows.
For a given target capacity $C$, we can partition the set of
$\mathcal{N}$ clients into two groups according to the PRPs from the
source to these nodes, then those nodes with PRPs above $C$ will be
selected as the relay nodes since they have residual capacities to
serve the remaining nodes.

The rational for selecting relay nodes in this way is that the
selected relay nodes can meet the target capacity requirement.
However, there is no guarantee that the remaining nodes can achieve
the target capacity $C$ too since their achievable throughput
depends on their link capacities to the relay nodes, as well as how
much residual time that the relay nodes can devote for cooperation.
Therefore, it is needed to check the feasibility of this target $C$,
which involves the computations of the available cooperation time
for a given set of relays (to be discussed), with which we can
compute the achievable throughput for each receivers. If any of the
nodes fail to achieve the target capacity $C$, then that means this
target is infeasible and a smaller one should be attempted,
otherwise a larger capacity may be supported.

Based on this idea, we propose a binary search procedure to find the
maximum achievable capacity as shown in
Algorithm~\ref{alg:relay_node_search}. The algorithm maintains two
thresholds for the target capacity, the lower threshold $C_{L}=0$
and the upper threshold $C_{U}=1$ initially. Starting from
$C=(C_{L}+C_{U})/2$, a set of relay nodes with qualified link
capacities (where $c_{0,k}$ denotes the link capacity between the source
and node $k$) is determined (lines 5-6). Then the achievable
capacities of the remaining nodes are computed using Algorithm 2
(line 7). If the target capacity can be satisfied by all nodes, then
the lower threshold is increased to $C$ (line 9), otherwise the
upper threshold is reduced to $C$ (line 11). The same procedure is
repeated until the upper and lower thresholds converge. Finally, the
algorithm can return  the set of qualified relay nodes for the
maximum achievable capacity $C^*$.

\begin{algorithm}[t]
\SetLine \Begin{
  $C_L \leftarrow 0, C_U\leftarrow 1$;

  \While {$C_U-C_L>\Delta$} {
  $C \leftarrow (C_U-C_L)/2$\;

  $\mathcal{N}_1 \leftarrow \{k|c_{0,k} \geq C, k\in \mathcal{N}\}$\ ;

  $\mathcal{N}_2 \leftarrow \mathcal{N}\backslash \mathcal{N}_1$\;

  Invoke Algorithm 2 to check the feasibility of $C$ for the partition of $\mathcal{N}_1$ and $\mathcal{N}_2$\;

  \uIf {$C$ is feasible} {$C_L \leftarrow C$;}
  \Else {$C_U \leftarrow C$;}
  }
} \caption{Relay Nodes Selection} \label{alg:relay_node_search}
\end{algorithm}

\subsubsection{Relay time allocation} As discussed in the previous subsection, for a target capacity $C$, if a node $i$ has a PEP of $c_{0,i} > C$,  it is selected as a candidate relay node. In this case, at least $C/c_{0,i}$ of its time has to be used for receiving data from the source so that the target capacity requirement can be satisfied. As a result, its residual time is at most $(c_{0,i}-C)/c_{0,i}$, which can be used for serving the remaining receiver nodes. Therefore, the next problem is to find the allocation of the relay time for each relay node under its residual time budget, such that all the receiver nodes can also meet the target capacity requirement. If such time allocation exists, it means the target capacity is achievable, and vice versa.

To this end, we propose a relay time allocation algorithm as shown
in Algorithm~\ref{alg:relay_time_allocation}, which proceeds in
round as follows. In the beginning, each candidate relay node $i\in
\mathcal{N}_1$ is initialized with the residual time $C_i =
(c_{0,i}-C)/c_{0,i}$ (line 2), and each receiver node $j\in
\mathcal{N}_2$ has a residual capacity demand $D_j = C$ (line 3). In
each round $l$, a greedy algorithm (ALG 3) is invoked to select a
subset $\mathcal{R}_l$ from $\mathcal{N}_1$ with at most $K-1$
elements, such that the overall capacity of all nodes in
$\mathcal{N}_2$ is maximized (line 7), where the capacity of a node
$j$ is determined as $c_{i',j}$ such that $i'$ is the node in
$\mathcal{R'}_l = \mathcal{R}_l\bigcup\{source\}$ with the maximum
capacity to node $j$ among all nodes in $\mathcal{R'}_l$.

Given the relay subset $\mathcal{R}_l$, the next step is to decide
the time ratio $\tau_l$ that they can devote for relaying.  Note
that since none of the relay nodes should contribute more than its
residual time, and none of the receiver nodes should get service
more than its residual capacity demand, so the rely time $\tau_l$
for this subset $\mathcal{R}_l$  is set to the minimum of the
residual time of these relay nodes and the residual demand of all
receivers (line 8). Then for each selected relay node $i$, its
residual time is reduced by the amount of $\phi_l$ (line 10). If its
residual time is used up, it is removed from the candidate relay set
and will not participate in the relay time allocation in the next
round (line 11). Similarly, for each receiver $j$, its residual
demand is reduced by an amount of $\phi_l*q_{i', j}$, which is the
effective throughput it will receive from this set of relay
nodes(line 14). If its demand is satisfied, it is removed from
receiver set and will be considered in the next round (line 15). The
same procedure is repeated to find the next subset of relay nodes
and its relay time allocation, until either the candidate relay set
$\mathcal{N}_1$ or the receiver set $\mathcal{N}_2$ becomes empty,
or the overall relay time reaches 1 (line 8). If the receiver set
$\mathcal{N}_2$ is empty eventually, it means that the target
capacity demand $C$ can be met by all receiver nodes, then the
algorithm returns a list of relay subset and their corresponding
relay time; Otherwise, it means the target capacity $C$ is
infeasible and the algorithm returns an empty set.

\begin{algorithm}[t]
\SetLine

%\KwIn{Target capacity $C$, candidate relay set $\mathcal{N}_1$, and receiver set $\mathcal{N}_2$;}
%\KwOut{A list of relay subset and relay time allocation $\{\mathcal{N}_l, \phi_l\}_{l\in \mathcal{L}}$;}

\Begin{
  $C_i \leftarrow (c_{0,i}-C)/c_{0,i}, \forall i \in \mathcal{N}_1$\;
  $D_j \leftarrow C, \forall j \in \mathcal{N}_2$\;
  $l \leftarrow 0$ \;
 \While{$\mathcal{N}_1 \neq \emptyset$ and $\mathcal{N}_2 \neq \emptyset$ and $\sum_l \phi_l \leq 1$} {
   $l \leftarrow l+1$\;
   Call Algorithm 3 to select a subset $\mathcal{R}_l \subseteq \mathcal{N}_1$ with $|\mathcal{R}_l|\leq K-1$, such that $\sum_{j\in \mathcal{N}_2} c_{i',j}$ is maximized, where
    $i' \leftarrow \arg \max_{i\in \mathcal{R}_l \bigcup \{source\}} c_{i,j}$\;

   $\phi_l \leftarrow \min\{\min_{i\in \mathcal{R}_l} C_i, \min_{j\in \mathcal{N}_2} D_j/c_{i',j}, 1-\sum \phi_i\}$\;

   \ForEach{$i \in \mathcal{R}_l$} {
        $C_i \leftarrow C_i - \phi_l$;

        \lIf {$C_i \leq 0$} {$\mathcal{N}_1 \leftarrow \mathcal{N}_1 \backslash i$;}
    }
   \ForEach{$j \in \mathcal{N}_2$}{

    $D_j \leftarrow D_j - \phi_l*c_{i',j}$;

    \lIf {$D_j\leq 0$} {$\mathcal{N}_2 \leftarrow \mathcal{N}_2\backslash j$;}
    }
 }
   \lIf {$\mathcal{N}_2 == \emptyset$} {\KwRet{$\{\mathcal{R}_l, \phi_l\}_{l\in \mathcal{L}}$}}\;
   \lElse {\KwRet{ $\{\emptyset\}$};}
 }

\caption{Relay Time Allocation} \label{alg:relay_time_allocation}
\end{algorithm}


In each round of Algorithm 2 (line 7), we need to find a subset of
at most $K-1$ relay nodes that can provide maximum capacity to the
unsatisfied receivers with the source. Let $\mathcal{B}$ denote the set nodes consisting of the relay candidate set $\mathcal{N}_1$ and $source$. Each node pair $(i,j), i\in \mathcal{B}, j\in \mathcal{N}_2)$ is associated a capacity $c_{i,j}$.  A selection is a tuple $S=(\beta,f)$, where $\beta$ is a subset of $\mathcal{B}$, and $f$ is an assignment function from $\mathcal{N}_2$ to $\beta$. The capacity of a selection $S$ is given by $C(S) =
\sum_{j\in \mathcal{N}_2} C_{f(j), j}$. 

This problem is a special case of
the class of Generalized Maximum Coverage Problem\cite{Cohen2008},
which can be formally described as follows:

Note that in our case, when $\beta$ is given, the best assignment
function $f$ is to map an receiver $R_j \in \mathcal{N}_2$ to the
station $R\in \mathcal{B}$ with the maximum capacity. So from now
on, a selection is simply denoted as $S=\beta$. This problem, known
as a special case of the generalized maximum coverage problem, is
NP-hard. Instead we develop a greedy approximation algorithm for
this problem similar to \cite{Cohen2008}. The basic idea is to
define the sender $R_i$'s residual capacity for a receiver $R_j$
which is previously selected to receive information from the
transmitter $R_{i'}$, which equals the capacity difference
$c_{i,j}-c_{i',j}$. The intuition behind the greedy algorithm is
that by adding a new transmitter to $\beta$, only the positive
residual profit can be gained.



\bfseries Definition 1 (residual capacity/weight) \normalfont
Consider a selection $S=(\beta)$, a relay $i\in S_A$, and a
second-layer receiver $j\in R_D$. We define the residual capacity
$R_S(i,j)$ to be equal to $c(i,j)-c(f(j),j)$.


\bfseries Definition 2 (addition of a relay) \normalfont For a
selection $S=(\beta)$ and a relay $i\not\in \beta$, we define
$S\oplus i$ as the addition of $i$ to $S$. Since $f$ always finds
best forwarder, for every station $j\in R_D$ we have:
\begin{eqnarray}
f^*(j)=\left\{
\begin{array}{ll}
i &when c_{i,j}>c_{f(j),j} \\
f(j) &otherwise
\end{array}
\right.
\end{eqnarray}



Base on this residual capacity concept, a greedy maximum coverage
algorithm is proposed in Algorithm~\ref{alg:greedy_coverage}. The
basic idea of this algorithm is to incrementally add relay node with
positive residual capacity, so that the overall capacity is
non-decreasing. At line 3, all receivers are initially assigned to
the source. Then in each round, one of the relays that has the maximum
positive residual capacity is chosen to be added in the relay node
sets (line 6) until $K$ channels have been occupied. This greedy
algorithm can be proved to achieve an approximation ratio
$1-(1-\frac{1}{K-1})^{K-1}$ to the optimal solution. The details of
the proof are given in the Appendix.

\begin{algorithm}[t]
\SetLine \Begin{
  $k \leftarrow 1$\;
  Assign all receivers in $\mathcal{E}$ to the source, i.e.,
  $f(e) \leftarrow source$ \;
  \While{$k\leq K$}{
   Pick a relay $R$ with the maximum residual capacity, i.e., $R\leftarrow \arg \max_{b'\notin \beta} R_S(b', E)$\;
   \lIf{$R_S(b, E) > 0$}{
   $\beta \leftarrow \beta \oplus b$\;
   $k \leftarrow k+1$\;
   }
   \lElse {break;}
  }
  \KwRet{$\beta$.}
} \caption{Greedy Maximum $k$-Coverage} \label{alg:greedy_coverage}
\end{algorithm}

\subsubsection{Online Relay Transmission Scheduling}
From Algorithms 1-2, we can find a list $\mathcal{L}$ of relay node
set $R_l$ and the corresponding relay time allocation $\phi_l$, such
that the multicast capacity of the system is maximized. Let $C^*$
denote the maximum capacity corresponding to this results, then for
any capacity requirement $C\leq C^*$, we should have:
\begin{equation}\label{eq:scheduling}
 C\leq \sum_{i'=\arg \max_{i\in \mathcal{R}_l\bigcup \{source\}} c_{i,j}, l\in \mathcal{L}} \phi_l*c_{i', j}, \forall j \in \mathcal{N}.
\end{equation}

From \eqref{eq:scheduling}, we can see that the amount of time that
a subset $\mathcal{R}_l$ to be scheduled for relaying should be
proportional to $\phi_l$, such that the required capacity can be
satisfied. Since the time is slotted, as briefly introduced in last
section, we can adopt a stochastic online algorithm to approximate
the scheduling. Specifically, let us define $\psi_l$ as
\begin{equation}
\psi_l = \sum_{k\leq l} \phi_l, \forall l.
\end{equation}

In each time slot $t$, the source generates a random number between 0
and 1, if its value falls between $\psi_k$ and $\psi_{k+1}$, then
the $k^{\text{th}}$ subset of relay nodes are selected for relaying
in this time slot. It is easy to see that this stochastic scheduling
policy converges to the required proportional of time for each relay
set in a long run. This schedule algorithm can be executed by the source
in an online fashion at the beginning of each time slot, and a
unique channel is assigned to each selected relay node. The
scheduling result (relay nodes and their operating channels) are
broadcasted to all receivers, then they can choose the best relay
node and switch to the corresponding channel for receiving the data.

